Federated Domain Adaptation for ASR with Full Self-Supervision

Cross-device federated learning (FL) protects user privacy by collaboratively training a model on user devices, therefore eliminating the need for collecting, storing, and manually labeling user data. While important topics such as the FL training algorithm, non-IID-ness, and Differential Privacy have been well studied in the literature, this paper focuses on two challenges of practical importance for improving on-device ASR: the lack of ground-truth transcriptions and the scarcity of compute resource and network bandwidth on edge devices. First, we propose a FL system for on-device ASR domain adaptation with full self-supervision, which uses self-labeling together with data augmentation and filtering techniques. The system can improve a strong Emformer-Transducer based ASR model pretrained on out-of-domain data, using in-domain audio without any ground-truth transcriptions. Second, to reduce the training cost, we propose a self-restricted RNN Transducer (SR-RNN-T) loss, a variant of alignment-restricted RNN-T that uses Viterbi alignments from self-supervision. To further reduce the compute and network cost, we systematically explore adapting only a subset of weights in the Emformer-Transducer. Our best training recipe achieves a $12.9\%$ relative WER reduction over the strong out-of-domain baseline, which equals $70\%$ of the reduction achievable with full human supervision and centralized training.

==> paper/abstract_ServerEmulatedFL.tex <==
\begin{abstract}
{Cross-device federated learning (FL) protects user privacy by performing training locally on user devices, therefore eliminating the need for collecting, storing, and manually transcribing user data. However, building practical cross-device FL for full-scale end-to-end automatic speech recognition systems presents many technical challengs.
%
%Some challenges lie in building a robust infrastructure for consenting and enrolling users, encrypting on-device data caching, enabling on-device ASR training and inference under resource constraints, and efficiently communicating on-device ASR gradients asynchronously to the FL server; other challenges are modeling-specific, which include the absence of ground truth ASR transcriptions, and ensuring the quality of FL on-device ASR models despite the non-IIDness of user updates.
%
These include robust user-consent infrastructure, encrypted on-device storage, resource-constrained ASR training, and gradient communication to the FL server. Other challenges are modeling-specific, such as the absence of ground truth ASR transcriptions, and ensuring the quality of FL on-device ASR models despite the non-IIDness of user updates.
%
To make progress on the modeling aspects for the cross-device FL in the absence of the robust infrastructure, we built a {\em server-emulated FL} system as an intermediate step, and present the empirical learnings on updating and training on-device streaming ASR models, gained with this server-emulated FL system.
We successfully improve a strong seed ASR model, originally trained on out-of-domain audio, with domain data without ground truth transcriptions, via the FedAvgM/BMUF training algorithm.
%
We identify two key components that we find necessary for the success of the semi-supervised learning scheme, namely data augmentation and confidence filtering.
%
Furthermore, in preparation for efficient on-device training and FL of the ASR models, we show that training only a subset of parameters not only is a viable mitigation to communication cost, but also improves accuracy.
%
The resulting system achieves a $12.9\%$ relative WER reduction over a strong out-of-domain baseline, and achieves $70\%$ of the gain achievable with full human supervision and data parallel training.
}
%
\end{abstract}
\noindent\textbf{Index Terms}: speech recognition, unsupervised domain adaptation, federated learning

==> paper/introduction_ServerEmulatedFL.tex <==
\section{Introduction}
%
With the growing adoption of deep neural networks (DNNs) in artificial intelligence applications, users are increasingly aware of data privacy concerns, since DNN models require large collections of field data druing training~\cite{mireshghallah2020privacy,ha2020security}.
%
Automatic speech recognition (ASR) is a particularly sensitive application, due to the personal nature of speech~\cite{schuller2013computational,cherkassky2021voice}.
%
To better protect user privacy, recent works developed cross-device Federated Learning for ASR applications~\cite{gao2021end,nandury2021cross,yu2021federated,guliani2021training,dimitriadis2020federated,cui2021federated}.

\cite{nandury2021cross} describes Federated Learning (FL) as a ``distributed training paradigm that allows a loose federation of trainers to collaboratively improve a shared model''~\cite{konevcny2016federated,mcmahan2017communication,li2021survey}.
In cross-device FL, these trainers run on individual user devices, thereby protecting users' privacy since no audio nor transcripts ever leave users' devices.

The most common FL setup can, in a nutshell, be described as akin to distributed training via hierarchical SGD with semi-supervised pseudo labels on data that are not independent and identically distributed (i.e. non-IID).
The hierarchical SGD method was first developed in the speech community under the name {\em blockwise model-update filtering}, or BMUF \cite{bmuf}). In the Federated-Learning community, the same algorithm has become known as {\em Federated Averaging with Momentum}, abbreviated as FedAvgM \cite{}).

Developing the complete cross-device FL stack for end-to-end production-scale on-device ASR models presents a broad range of challenges with respect to both infrastructure and ASR modeling. It requires robust infrastructure support for consenting and enrolling users; encrypted temporary on-device data storage; enabling on-device ASR; as well as efficient and secure communication of on-device-created ASR gradients asynchronously to an FL server. At the same time, for ASR, one has to deal with hierarchical SGD over extremely slow networks; the absence of ground truth ASR training transcriptions; ensure the quality of FL on-device ASR models despite the non-IID-ness of user updates, and mitigate potential accuracy regressions due to the use of differential privacy.

Hence, while our ultimate goal is on-device FL in a cross-device setting, we break the complex problem up and aim at taking an intermediate step where we emulate the FL algorithms inside our existing cloud-based ASR service. In what we call {\em Server-Emulated FL}, we aim to use our ASR servers as ``devices'' as a testing ground. In this role, ASR servers compute local BMUF model updates as part of serving ASR requests. Only aggregated model updates are then sent to a central FL server for aggregation.

In this work, we share practical learnings in a number of modeling-related aspects gained in the development of this intermediate step of Server-Emulated FL.

% In this work, we assume a cross-device FL setting, in which each device stores a limited history of its own user data in an encrypted cache and computes local model updates using the data. Only model updates are sent to a central FL server for aggregation. 
%
We identify two main modeling challenges for the server-emulated FL ASR training.
%
First, the lack of ground truth labels. While past work has frequently assumed the availability of ground-truth transcriptions when training ASR with FL~\cite{gao2021end,yu2021federated,guliani2021training,dimitriadis2020federated,cui2021federated}, this is not realistic. Users of on-device ASR applications generally do not correct inaccurate transcriptions for their own utterances; FL is limited to pseudo labels of unknown quality.
Secondly, catastrophic forgetting. In cross-device FL, the quality of the ASR should not degrade drastically for the long tail (or at all) after adapting to each device's own user data. It is also undesirable to communicate the entire model back and forth between devices, as the cost of communication (especially the uplink to send gradients back) dominates~\cite{konevcny2016federated}. This is despite the fact that in an actual on-device cross-device FL, devices only participate in FL when plugged in and communicating on unmetered WIFI networks~\cite{mcmahan2017communication}. 


% In this work, we consider a realistic cross-device FL system, where an ASR application runs locally on users' devices, and we improve the global shared ASR model with FL.

%
% Privacy is protected because no user audio, nor transcripts, ever leave their device.
%
% Very few works, however, addressed the challenges of building a cross-device FL system for ASR. 

% In this work, we consider a realistic scenario where an ASR service provider runs their ASR model locally on user devices, such as wearables, and manages a FL system to improve a global shared ASR model.
% %
% A user may choose to participate in FL, which would grant permission to setup a trainer on their device, use their data for computing local model updates, and periodically send model updates (but no audio or transcripts) to the central FL server.
% %
% The success of FL in such a scenario depends on the effectiveness of the learning method as well as user willingness to participate in FL.

% Existing works fail to address the practical challenges in such a realistic scenario.
%
% First, most existing works assume the availability of ground truth transcriptions~\cite{gao2021end,yu2021federated,guliani2021training,dimitriadis2020federated,cui2021federated}.
%
% This is unrealistic because ASR users generally do not transcribe or correct their own audios.
%
% Second, we are not aware of existing work [TODO: sure?] that investigated how to reduce the costs of training and communicating the ASR model.
%
% However, in reality many devices have slow internet connection (esp.~the uplink), while state-of-the-art ASR models contain at least tens of millions of parameters and are computationally intensive to train. 
%
% [TODO: We do not address computation in this paper. Let's remove that everywhere.]
% %
% As such, naively training and communicating the entire ASR model would consume too much computation resource and internet bandwidth, therefore discourage user participation in FL.

\begin{figure}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{LaTeX/figs/overview.pdf}
    \caption{Semi-supervised Federated Learning system, in its intermediate incarnation of {\em server-emulated FL} where the role of ``devices'' is played by ASR servers.}
    \label{fig:overview}
\end{figure}

We show that despite these challenges, it is possible to successfully improve a strong ASR model, which was pre-trained on large amounts of out-of-domain audio, and updated with users' on-device data via the BMUF algorithm (more commonly known as FedAvgM). To the best of our knowledge, this work is novel in that we tackle the lack of ground-truth transcription using semi-supervised learning method for a streaming on-device ASR model. In particular, we develop a novel set of techinques to utilize the existing on-device ASR model to label and align locally aggregated data, and then apply data augmentation and confidence-score flitering to construct a subset of training data on-device. 
[TODO: Now this needs to be reconciled with server-emulated.]
%
Moreover, to ensure that the ASR model updates could be efficiently communicated between device and FL server, we demonstrate that training only a subset of parameters successfully mitigates the communication costs. In fact, it can also improve the accuracy of the resulting FL-trained model.
%
Via these methods, we
achieve a XXX\% relative WER reduction over a strong out-
of-domain baseline -- YY\% of the gain achievable
with full human supervision and data parallel training.

Many past works have also addressed similar challenges. Most simliar to our work, Tsouvalas et al.~\cite{tsouvalas2021federated} developed semi-supervised FL for ASR by leveraging the existing on-device ASR model to do self-label on input transcripts. XXXXX (explain why it's different from our work)... In 



\textcolor{blue}{
[
Missing related works, here is a very rough list\\
\begin{enumerate}
    % Juteng: Thanks for finding those references! @June
    % \item similar to "Federated learning: Strategies for improving communication efficiency"  where subset of weights are updated using mask
    %Junteng: this work use random masking which I believe the primal team tried that did not work (need to confirm with Jay), our work use a fixed group of weights for finetuning (maybe more specific to transformer transducer)
    % \item introduce 'Communicationefficient learning of deep networks from decentralized data' if needed
    \item Most similar work is "Federated Self-Training for Semi-Supervised Audio
Recognition" https://arxiv.org/pdf/2107.06877.pdf where they used self-leanring to show results on ASR. 
    \item Another simlar to Apple's on-device ASR personalization paper https://arxiv.org/pdf/2102.08503.pdf where they used semi-supervised self labeling for ASR personalization.    
    %Junteng: correct me if I am wrong, I think they proposed SSL idea but did not try; also they did not use self-supervision
    \item "SSFL: TACKLING LABEL DEFICIENCY IN FEDERATED
LEARNING VIA PERSONALIZED SELF-SUPERVISION" non-speech related :  https://arxiv.org/pdf/2110.02470.pdf
\item 
\end{enumerate}  ]}


In Section~\ref{sec: method}, we first elaborate on our server-emulated FL system setup. In Section~\ref{subsec:effectiveness}, we explain our approaches to make cross-device FL ASR work with unlabeled user data efficiently. We explained our data and experimental set up in Section~\ref{sec:experiments}, followed by results and conclusion~\ref{sec:conclusion}. 


% On a high level, we first train an initial ASR model on public available data with ground truth transcriptions or high-quality pseudo labels. We then use Federated Learning on semi-supervised pseudo labels to adapt the pretrained model to users' data on their devices. In particular, we design the FL model updates to be part of the ASR on-device application. 
%
% In particular, the trainer runs alongside the ASR service in the same container.
%
% When ASR requests are completed, we provide the audios and the ASR output transcriptions to the FL trainer for computing local model updates.
% 
%
%
% If each container is a user device, then this is exactly a cross-device FL system.
%
% However, here we take a step back and consider building an intermediate system where each container is an ASR server hosted in the cloud, and we refer this as a server-emulated FL system.
%
% There are a few reasons why such an intermediate system is valuable.
%
% First, a cross-device FL system is extremely difficult to setup and requires user consents to use their device for training.
%
% The server-emulated FL allows leveraging existing infrastructures of the ASR service to perform online testing of FL in a simulated environment.
%
% Second, the server-emulated FL system already provides effective privacy protections on its own.
%
% Since no human transcription is needed, learning can be performed on-the-fly and user data does not need to be stored.
%
% Furthermore, access control can be implemented between the ASR servers and the service provider to ensure no accidental leakage of user data.
%
% One example use case of the server emulated FL system is for improving live video captioning in online streaming services, where storing user data is neither necessary nor desired.

% We report some important learnings from building the server-emulated FL system, taking the transformer transducer as the ASR architecture~\cite{gulati2020conformer,shi2021emformer}.
%
% Our conclusions can be summarized as follows:
% %
% 1) Semi-Supervised domain adaptation is effective in the federated learning setting, and data augmentation and confidence filtering are the keys to its success.
% %
% 2) We can greatly reduce the computation and communication cost without hurting the FL performance, by modifying the RNN-T loss function and finetuning on a selected subset of parameters.
% %
% Those learnings are very valuable for building a realistic cross-device FL system for improving the ASR model in the future.

%\textcolor{red}{[TODO: mention non-iidness as one of the challenges, stress that we focus on things not yet addressed by others; that our finding is complementary to existing works]}
